Improving Semantic Embedding Consistency by Metric Learning for Zero-Shot Classification

This paper addresses the task of zero-shot image classification. The key contribution of the proposed approach is to control the semantic embedding of images -- one of the main ingredients of zero-shot learning -- by formulating it as a metric learning problem. The optimized empirical criterion associates two types of sub-task constraints: metric discriminating capacity and accurate attribute prediction. This results in a novel expression of zero-shot learning not requiring the notion of class in the training phase: only pairs of image/attributes, augmented with a consistency indicator, are given as ground truth. At test time, the learned model can predict the consistency of a test image with a given set of attributes , allowing flexible ways to produce recognition inferences. Despite its simplicity, the proposed approach gives state-of-the-art results on four challenging datasets used for zero-shot recognition evaluation.

==> 8-reviews.tex <==

\clearpage
\section{reviews}
\begin{itemize}
\item[R1] "(1) Correctness of claims of novelty is not clear."
\begin{itemize}
\item Akata et al, "Attribute Label Embedding" [29] and Romera Paredes et al, "Embarrassingly Simple .." [2] are recent well known papers with very similar ideas to the ones proposed here. While these are discussed in Ln 162 167, it is not explained what conceptual novelty the proposed method has, when compared to these. {\bf [corrig\'e mais \`a v\'erifier.]}
\item The claim of novelty from being the first to use metric learning for the zero shot problem (Ln 225) is overstated and does not do justice to prior work. Mensink et al. [51] (uncited reference), Weston et al, "WSABIE.." (IJCAI 2011) and are well known papers that also use metric learning for zero shot problems. WSABIE in particular is highly cited and has inspired several other methods for zero shot learning, including [29] and [2] from the above point. A quick google search for "metric learning zero shot" brings up several more relevant references such as Zhang, "Joint Latent Similarity Embedding", Kuznetsova, "View Specific Appearance Similarities". {\bf [corrig\'e mais \`a v\'erifier.]}


\item include results from Table 2 of Zhang, "...Joint Latent Similarity Embedding" {\bf[ok]}
\end{itemize}
\item[R1] (2) In general, relationship to prior work should be made much clearer throughout. Another instance:
\begin{itemize}
\item Related work(Ln 237): "However, in contrast to our work, [38] do use class label in the training process, which makes it a [sic] the end, very close to [21]". This statement is (i) vaguely worded, (ii) dismissive and implies a wrong ordering of [38] and [21], and also (iii) overstates the value of class labels, given that attribute labels are known. (i) The oldest methods like DAP do not require class labels during training either. (ii) Class labels are pretty strongly associate with distinct attribute signatures. This is the whole premise of zero­shot learning with attributes, after all. In fact, for datasets like AwA with class­level attribute annotations, knowing the attributes is *exactly equivalent* to knowing the class label. (iii) Even ignoring (ii), the class label is only one extra annotation over the many attribute annotations.

\item In general, all subsections of Section 2 (Related work) would strongly benefit from statements indicating clearly how this work relates to the literature, esp. given my point (1) relating to novelty above.
\end{itemize}
\item[R1]  Lack of clarity in writing * proofreading * here are a few examples that I found particularly difficult to understand:\\ ­ Ln 325: "resulting metric takes into account the informational data structure, typically discriminant relationships." ("informational data structure"? "discriminant relationships"?) {\bf[ok, correction proposee rebuttal]} \\ Ln 322: "the link between class and attribute representation is assumed given by the application context" ("application context"?) {\bf[ok, correction proposee rebuttal]}\\ Ln 333: "the exploitation of pairs of data is expected to catch the specific way of being similar and dissimilar in the actual data distribution" (I don't understand this) {\bf[ok]}\\ In intro, trying to describe the main novelty of the paper:  Ln 45-60: "recent trends in ZSL studies are aiming at controlling classification inference as well as the attribute prediction in the learning criteria ... In the work proposed in this paper, we instead suggest that better controlling the structure of the sole embedding attribute space is at least as important than constraining the classification inference step." >>>>>What is "sole embedding" here? (ctd.){\bf[ok]}\\ "More specifically, we use a ... allowing balance between attribute prediction and discriminating capacity" >>>>>This sounds like the same thing as the "recent trends" description above. {\bf[ok]}

\item Please list final hyperparameter values for reproducibility (Ln 462) 
\item Table 3: The improvements over [11] are very strong for other columns, but there is a significant drop for SUN alone. Any insight into why this (both the improvements and the might this be the case? ­ 
\item Ln 157: "DAP vs IAP"  please see the journal version of [3] that shows this not to be the case any longer 
\item[R1]  Many uncited references [46-61]. Mistake? {\bf [corrig\'e.]}  
\item[R2] (1) The notation of the paper contains quite some issues. Several of them are listed below.\\ In line 319, the similarity S is unknown in training, the training pair should be $(\mathbf{X}_i,\mathbf{Y}_i)$ {\bf [corrig\'e.]} \\ In line 331 and 332, $\mathbf{X}$ and $\mathbf{Y}$ should be $\mathbf{X}_i$ and $\mathbf{Y}_i$. : {\bf [corrig\'e.]} \\ In line 384, the attribute class descriptor should be ${\mathbf{Y}*_k}_{k = 1}^{C}$, C is the number of the classes. {\bf [corrig\'e.]} \\ In line 401, bold letter should be used. {\bf [corrig\'e.]} 
\item[R1] readability of  figures not good /  line  too thin + legend too small. {\bf [limite de 14 pages, ok sur \'ecran]}
\item[R2] The proposed method has 4 hyper-parameters. The authors recommended to do a grid search to determine the values. The authors should clearly illustrate the search range  {\bf [corrig\'e.]} and step in the manuscript and show whether the algorithm is stable in terms of them.
\item[R3] taking into account multi task learning view on the attribute levels (for example: Predicting Multiple Attributes via Relative Multi­task Learning, CVPR 2014) using for example multi task metric learning framework of Large Margin Multi­Task Metric Learning, NIPS 2010. {\bf [corrig\'e. j'ai remplac\'e le terme multi-task par multi-objective.] }
\item[R3] add running times {\bf [corrig\'e.]}
\end{itemize}


